Anti-Adversarially Manipulated Attributions for Weakly Supervised Semantic Segmentation and Object Localization

Obtaining accurate pixel-level localization from class labels is a crucial process in weakly supervised semantic segmentation and object localization. Attribution maps from a trained classifier are widely used to provide pixel-level localization, but their focus tends to be restricted to a small discriminative region of the target object. An AdvCAM is an attribution map of an image that is manipulated to increase the classification score produced by a classifier before the final softmax or sigmoid layer. This manipulation is realized in an anti-adversarial manner, so that the original image is perturbed along pixel gradients in directions opposite to those used in an adversarial attack. This process enhances non-discriminative yet class-relevant features, which make an insufficient contribution to previous attribution maps, so that the resulting AdvCAM identifies more regions of the target object. In addition, we introduce a new regularization procedure that inhibits the incorrect attribution of regions unrelated to the target object and the excessive concentration of attributions on a small region of the target object. Our method achieves a new state-of-the-art performance in weakly and semi-supervised semantic segmentation, on both the PASCAL VOC 2012 and MS COCO 2014 datasets. In weakly supervised object localization, it achieves a new state-of-the-art performance on the CUB-200-2011 and ImageNet-1K datasets.

==> Figures/cub_bg_suppress_summary.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{Figures/bg_suppress_fig_v3_print.pdf}
\vspace{-1.5em}
\caption{\label{fig_bg_suppress_summary} \rv{Two examples showing (left-hand images) the suppression of (normalized) attribution scores in background regions of an image; and (right-hand images) the sorted distribution of attribution scores of each pixel in the corresponding CAM and AdvCAM. The blue boxes represent ground truth, and the green boxes represent predictions.}}
\end{figure*}


==> Figures/grad_sample_summary.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{Figures/grad_sample_v2.pdf}
% \vspace{-2.3em}
\caption{\label{grad_sample} Examples of visual saliency maps~\cite{simonyan2013deep} of manipulated images at $t=0$, $t=5$, $t=10$, and $t=20$. The red box represents the target object.
}
\vspace{-1em}
\end{figure}


==> Figures/per_year_gain.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figures/per_year_altogether_v2.pdf}
% \vspace{-2em}
\caption{\label{peryeargain} Increases in best mIoU achieved with the PASCAL VOC 2012 validation images from 2019 to 2021, (a) with saliency supervision and (b) without saliency supervision. Also, Top-1 localization accuracy \textit{vs.} MaxBoxAccV2@IoU0.5~\cite{choe2020evaluation} for recent methods on (c) CUB-200-2011 and (d) ImageNet-1K.}
% \vspace{-1em}
\end{figure}


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Tables/maxboxacc.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
\normalsize
% \renewcommand{\arraystretch}{1.2}
  \centering
  \caption{Comparison of Top-1 classification accuracy and \texttt{MaxBocAccV2} with CutMix~\cite{yun2019cutmix} and our method on the ImageNet and CUB-200-2011 datasets. ResNet 50.}
    \begin{tabular}{l@{\hskip 0.5in}cccc}
    \Xhline{1pt}\\[-0.95em]
    \multicolumn{1}{l}{\multirow{2}[0]{*}{Method}} & \multicolumn{1}{c}{Top1-Cls} & \multicolumn{3}{c}{\texttt{MaxBocAccV2}@IoU} \\
    % \midrule
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Acc (\%)} & 0.3   & 0.5   & 0.7 \\
    \hline\hline 
    \\[-0.9em]
    \multicolumn{5}{l}{Dataset: CUB-200-2011} \\
    Ki \textit{et al.}~\cite{ki2020sample}  &   &    &       &       \\
    CutMix~\cite{yun2019cutmix} &   &    &       &       \\
    Ours  &       &       &       &  \\
    \multicolumn{5}{l}{Dataset: ImageNet} \\
    Ki \textit{et al.}~\cite{ki2020sample}  &   &    &       &       \\
    CutMix~\cite{yun2019cutmix} &   74.4    &    83.1    &   63.6    & 39.7  \\
    Ours  &       &       &       &  \\
    \Xhline{1pt}
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> Tables/table_figure_failure_together_summary.tex <==
\begin{table*}[t]
  \centering
  
\begin{minipage}{0.7\linewidth}
\normalsize
  \centering
  \includegraphics[width=1\linewidth]{Figures/pami_revision_failure_v4.pdf}
  \vspace{-2em}
  \captionof{figure}{\label{fig_failure} \normalsize \rv{Failure examples for each dataset. For (c) and (d), the blue box represents the ground truth, and the green box represents the prediction. }}

  \end{minipage}\hfill
%   Table2

\begin{minipage}{0.7\linewidth}
\center
{\normalsize
\vspace{1em}
\color{red}
\begin{tabular}{l@{\hskip 0.in}c@{\hskip 0.1in}c@{\hskip 0.1in}c}
    \Xhline{1pt}\\[-0.95em]
    Method  & Precision & Recall & F1-score \\
    \hline\hline 
    \\[-0.9em]
    IRN$_{\text{~~CVPR '19}}$~\cite{ahn2019weakly} & 66.0  & 66.4  &   66.2 \\
    Chang \textit{et al.}$_{\text{~~CVPR '20}}$~\cite{chang2020weakly} &  61.0 & 77.2  &   68.1 \\
    SEAM$_{\text{~~CVPR '20}}$~\cite{wang2020self} & 66.8  & 76.8  &   71.5 \\
    AdvCAM (Ours)   & 66.9  & 77.6  & 71.9  \\
    AdvCAM--Sal (Ours) & \textbf{71.8} &  \textbf{78.2} & \textbf{74.9} \\

    % \\[-0.9em]
    \Xhline{1pt}
    \end{tabular}%
    }
    \vspace{0.2em}
      \caption{\rv{Comparison of precision, recall, and F1-score on the \rv{PASCAL VOC 2012} train images.}}
      \label{table_precrecall}%

  \end{minipage}\hfill

\end{table*}

==> Tables/table_prec_recall.tex <==
\begin{table}[t]
% \renewcommand{\arraystretch}{0.95}
\centering
\normalsize
  \caption{\rv{Precision recall. Pascal VOC}\label{table_precision_recall}}
%   Level of supervision: $\mathcal{F}-$full, $\mathcal{I}-$image label, $\mathcal{B}-$box, $\mathcal{S}-$saliency.}  
\vspace{-0.7em}
\color{blue}
\begin{tabular}{l@{\hskip 0.2in}ccc}
    \Xhline{1pt}\\[-0.95em]
    Method  & Precision & Recall & F-Score \\
    \hline\hline 
    \\[-0.9em]
    IRN$_{\text{~~CVPR '19}}$~\cite{ahn2019weakly} & 66.0  & 66.4  &   66.2 \\
    Chang \textit{et al.}$_{\text{~~CVPR '20}}$~\cite{chang2020weakly} &  61.0 & 77.2  &   68.1 \\
    SEAM$_{\text{~~CVPR '20}}$~\cite{wang2020self} & 66.8  & 76.8  &   71.5 \\
    AdvCAM (Ours)   & 66.9  & 77.6  & 71.9  \\
    AdvCAM--Sal (Ours) & \textbf{71.8} &  \textbf{78.2} & \textbf{74.9} \\

    % \\[-0.9em]
    \Xhline{1pt}
    
    \end{tabular}%
    
    % \end{adjustbox}
    \vspace{-1em}

      \end{table}

==> Tables/table_size_precisionrecall_coco_summary.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{\rv{Precision, recall, and F1-score averaged across all classes, the smallest 10 classes, and the largest 10 classes. All the results are computed for 6\% of the mages from the MS COCO 2014 dataset ($\approx$ 5000 images). The average sizes for each class were borrowed from the work of Choe \textit{et al.}~\cite{choe2020attention}.}}
  \begin{adjustbox}{width=1\textwidth}
  \normalsize
    \color{red}
  
    \begin{tabular}{l|ccc|ccc|ccc}
    \Xhline{1pt}
          & \multicolumn{3}{c|}{Total Classes} & \multicolumn{3}{c|}{Smallest 10 classes} & \multicolumn{3}{c}{Largest 10 classes} \\
        %   \\[-0.95em]\cline{2-10}\\[-0.95em]
          & Precision & Recall & F1-score & Precision & Recall & F1-score & Precision & Recall & F1-score \\
          \hline\hline
    CAM   &   44.5    &    61.6   &    47.6   & 11.5      &  \textbf{73.0}     &    19.2   &    69.3   &     60.4  & 63.5 \\
    AdvCAM ($T$=10, $\tau$=0.5) &   46.7    &   63.8    &     50.6  &  14.8     &     69.7  &     23.8  &    70.9   &    63.9   & 65.6 \\
    AdvCAM ($T$=20, $\tau$=0.5) &   47.1    &   \textbf{64.7}    &    51.3   &   16.5    &   67.4    &   25.4    &  70.9     &  \textbf{66.0}     & 66.5 \\
    AdvCAM ($T$=30, $\tau$=0.5) &    \textbf{48.1}   &    63.6   &    \textbf{51.6}   &  18.5    &  64.9     &   27.2   &   71.4    &    65.7   &  \textbf{66.7}\\
    AdvCAM ($T$=30, $\tau$=0.4) &  48.0     & 63.6      &   51.4    &     17.1  & 66.6      & 26.1      &    \textbf{71.5}   &  64.9     & 66.3 \\
    AdvCAM ($T$=30, $\tau$=0.6) &    47.7   &    63.7   &   51.4    &   \textbf{19.2}    &   64.3    &   \textbf{28.1}    & 71.2      &   66.1    & 66.5 \\
    \Xhline{1pt}
    \end{tabular}%
  \label{tab_size_pr_summary}%
  \end{adjustbox}
\end{table*}%

